SPOTS: An Accelerator for Sparse Convolutional Networks Leveraging Systolic General Matrix-Matrix Multiplication

This paper proposes a new hardware accelerator for sparse convolutional neural networks (CNNs) by building a hardware unit to perform the Image to Column (IM2COL) transformation of the input feature map coupled with a systolic array-based general matrix-matrix multiplication (GEMM) unit. Our design carefully overlaps the IM2COL transformation with the GEMM computation to maximize parallelism. We propose a novel design for the IM2COL unit that uses a set of distributed local memories connected by a ring network, which improves energy efficiency and latency by streaming the input feature map only once. We propose a tall systolic array for the GEMM unit while also providing the ability to organize it as multiple small GEMM units, which enables our design to handle a wide range of CNNs and their parameters. Further, our design improves performance by effectively mapping the sparse data to the hardware units by utilizing sparsity in both input feature maps and weights. Our prototype, SPOTS, is on average 1.74X faster than Eyeriss. It is also 78X, and 12X more energy-efficient when compared to CPU and GPU implementations, respectively.

==> extra-im2col.tex <==
Exploiting locality of accesses.

As explained in the background and motivation section, there are two sources of localities to exploit; spatial and temporal localities resulting from the overlap as the filters slide across different positions in the input feature map vertically and horizontally. Our PU organization is designed to take advantage of both localities to avoid accessing the same data multiple times to build different patches. 

Neighbor and Reserved Buffers.
Each PU is equipped with three buffers; the two buffers, neighbor, and reserved buffer are deployed to enable data reuse. The neighbor buffer stores the data received from the neighbor PU to exploit the spatial locality between the patches as we slide the filter across the input horizontally. The reserved buffers that keep the data will be used to build the future patches as the filter slides across the input vertically.     
 

Buffer Sizes.
The upper bound for each buffer can be calculated given the layer's features such as width, height, number of channels, kernel size, and stride size as follow. 

Size of the new buffer. The upper bound for the number of elements stored in the new buffer is kernel_size * kernel_size which belongs to the very first patch (top left). Most of the CNNs have a small kernel size of less than 5. But there are very few layers in some CNNs that have filters with kernel sizes larger than 10.  (Look at Table 2)

Size of the neighbor buffer. The kernel size and stride size dictate the overlap between the patches.  There will be an overlap between the two patches if the stride size is smaller than the kernel size. The number of elements shared between the two patches for one input channel is calculated as K*K - K*S. 

Size of the reserved buffers. The kernel slides across the input vertically. These cause some overlap between the two vertically adjacent patches. We store some of the elements in the reserved buffer to take advantage of vertically's localities. The accumulative total number of elements for a given filter size can be calculated as  number_of_channel * width * (Kernel_size-stride_size). Commonly, the width and number of channels are changing in opposite ways. In other words, earlier layers often have a small number of channels with larger input width. But, as we go to the bottom layers, the number of channels increases while the width gets smaller. As a larger having a buffer of size 32 KB, which we use for SPOTS, is sufficient to store almost all layers with different characteristics.   

What happens if the requirement exceeds the size of the reserved buffer?
We can skip using the reserved buffer altogether if a layer requirement exceeds the reserved buffers' size.  In those scenarios, some of the elements are accessed multiple times, and the data reusability will be limited to the horizontally adjacent patches.  

==> fig.im2colshare.tex <==
\begin{figure}[th]
  \centering
  \includegraphics[width=0.5\textwidth,angle=0]{./figures/im2colvsgemm.pdf}
\caption{\small Fraction of the work performed by the \imcol unit when
  compared to GEMM (i.e., GEMM bar is 100\%). We report the average and
  the median for the \imcol's work.  When the mean exceeds the median,
  there will be instances where the \imcol does significantly more work
  compared to GEMM for some layers.}
\label{fig:im2colvsgemm}
\end{figure}


==> fig.software.im2col.tex <==
\begin{figure}[th]
  \centering
  \includegraphics[width=0.5\textwidth,angle=0]{./figures/software_im2col.pdf}
\caption{\small Speedup with SPOTS over the software-based \imcol as the baseline.}
\label{fig:im2colsoftware}
\end{figure}

==> tab-sparse-format.tex <==

\begin{table}[t]
\centering
\caption{Comparison of percentages.}
\begin{tabular}{c|*2c|*2c}
\toprule
Model &  \multicolumn{2}{c}{Random} & \multicolumn{2}{c}{Block}\\ 
\midrule
{}   & Density   & Size  & Density   & Size \\ 
AlexNet   &  17.5 & 19.1   & 17.5  & 19.1\\ 
GoogleNet   &  11.8 & 12.7   & 29.3  & 31.9\\ 
VGG16   &  6.6  &  5.6   & 35.9  & 37.4\\ 
\bottomrule
\end{tabular}
\caption{Comparing the block pruning with random pruning in term of density and size of the network.}
\label{table:accuracynetwork}
\end{table}
